Asynchronous Collaborative Autoscanning with Mode Switching for Multi-Robot Scene Reconstruction

When conducting autonomous scanning for the online reconstruction of unknown indoor environments, robots have to be competent at exploring scene structure and reconstructing objects with high quality. Our key observation is that different tasks demand specialized scanning properties of robots: rapid moving speed and far vision for global exploration and slow moving speed and narrow vision for local object reconstruction, which are referred as two different scanning modes: explorer and reconstructor, respectively. When requiring multiple robots to collaborate for efficient exploration and fine-grained reconstruction, the questions on when to generate and how to assign those tasks should be carefully answered. Therefore, we propose a novel asynchronous collaborative autoscanning method with mode switching, which generates two kinds of scanning tasks with associated scanning modes, i.e., exploration task with explorer mode and reconstruction task with reconstructor mode, and assign them to the robots to execute in an asynchronous collaborative manner to highly boost the scanning efficiency and reconstruction quality. The task assignment is optimized by solving a modified Multi-Depot Multiple Traveling Salesman Problem (MDMTSP). Moreover, to further enhance the collaboration and increase the efficiency, we propose a task-flow model that actives the task generation and assignment process immediately when any of the robots finish all its tasks with no need to wait for all other robots to complete the tasks assigned in the previous iteration. Extensive experiments have been conducted to show the importance of each key component of our method and the superiority over previous methods in scanning efficiency and reconstruction quality.

==> figures/ablation-results.tex <==
\begin{figure}[t]
\centering
\subfigure[
]{
\begin{minipage}[t]{0.495\linewidth}
\centering
\includegraphics[width=\linewidth]{images/ablation-results-1.jpg}
%\caption{fig2}
\end{minipage}
}%
\subfigure[
]{
\begin{minipage}[t]{0.495\linewidth}
\centering
\includegraphics[width=\linewidth]{images/ablation-results-2.jpg}
%\caption{fig2}
\end{minipage}
}%

\subfigure[
]{
\begin{minipage}[t]{0.495\linewidth}
\centering
\includegraphics[width=\linewidth]{images/ablation-results-3.jpg}
%\caption{fig2}
\end{minipage}
}%
\subfigure[
]{
\begin{minipage}[t]{0.495\linewidth}
\centering
\includegraphics[width=\linewidth]{images/ablation-results-4.jpg}
%\caption{fig2}
\end{minipage}
}%
\centering
\caption{The evaluation results of efficiency (top row) and quality (bottom row) on the ablation studies over four virtual scenes. }
\label{fig:ablation-results}
\end{figure}

==> figures/comparisions-to-dong.tex <==
\begin{figure}[t]
\centering
\subfigure[ 
]{
\begin{minipage}[t]{0.495\linewidth}
\centering
\includegraphics[width=\linewidth]{images/compare-to-dong-1.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[ 
]{
\begin{minipage}[t]{0.495\linewidth}
\centering
\includegraphics[width=\linewidth]{images/compare-to-dong-2.png}
%\caption{fig2}
\end{minipage}
}%
\centering
\caption{Comparisons between our method and the work of \cite{dong2019multi} over four virtual scenes. }
\label{fig:compare-to-dong}
\end{figure}


==> figures/coverage-rate.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/coverage-rate.png}
  \caption{
    Ablation studies on the average scene recovery rate over ten virtual scenes.}
  \label{fig:coverage-rate}
\end{figure}

==> figures/distance-estimate.tex <==
\begin{figure}[htbp]
\centering
\subfigure[
]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.8in]{images/distance-estimate-2.pdf}
%\caption{fig2}
\end{minipage}
}%
\subfigure[
]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=1.8in]{images/distance-estimate-1.pdf}
%\caption{fig2}
\end{minipage}
}%
\centering
\caption{Illustration of the distance-estimation method.
To estimate the required travel distance in practice as (a) shows, 
we seek the barycenter of the viewpoints and calculate the traveling distance between the robot and the barycenter. 
The final estimation is the sum of the distance above and the distances from the barycenter to all candidate viewpoints, as (b) shows. 
}
\label{fig:distance-estimate}
\end{figure}

==> figures/intro-mist.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/intro-mist.pdf}
    \caption{
        An illustration of multiple robots scanning in an unknown environment. The dark mist in the top figure refers to the unexplored area.
        Three robots are scanning this indoor scene.
        Two of them are doing the reconnaissance job as "\rev{explorer}" (a) to broaden the known, and one robot is reconstructing the objects as a "\rev{reconstructor}" (b).
        The movement of robots (the green dots) and geometry information are all included in the global map (c).
        The control center makes further decisions according to this information.
    }
    \label{fig:intro-mist}
\end{figure}

==> figures/rms-colormap.tex <==
\begin{figure}[h]
   \centering
   \subfigure{
      \includegraphics[width=\linewidth]{images/reality-result.pdf}
   }
   \caption{
      \rev{Comparison between \cite{dong2019multi} and ours on relative RMS metrics. We compare the RMS per point in the final results, the color bar denotes differences of RMS between two methods. Red means \cite{dong2019multi} has higher RMS error while the blue one means the opposite. }
      % More reality reconstruction results using our method.
      % Objects with different semantic categories are in different colors. 
   }
   \label{fig:rms-colormap}
\end{figure}

==> figures/robot-num-ablations.tex <==
\begin{figure*}[htbp]
\centering
\subfigure[Total distance of S1
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-1.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[Total distance of S2
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-2.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[Total distance of S3
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-3.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[Total distance of S4
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-4.png}
%\caption{fig2}
\end{minipage}
}%

\subfigure[Time consumption of S1
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-5.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[Time consumption of S2
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-6.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[Time consumption of S3
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-7.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[Time consumption of S4
]{
\begin{minipage}[t]{0.245\linewidth}
\centering
\includegraphics[width=\linewidth]{images/robot-num-ablations-8.png}
%\caption{fig2}
\end{minipage}
}%
\centering
\caption{We evalutate our method with different number of robots with some of our ablation study terms. }
\label{fig:robot-num-ablations}
\end{figure*}

==> figures/tab_compare-to-dong-quality.tex <==
\begin{table}[]
\centering
\begin{tabular}{cccc}
\toprule
Method & ScCo & Recall\#1 & Recall\#2 \\ \hline \hline
Dong   &   85.83\%  & 45.51\%     &   63.82\%   \\
Ours   &   \bf{89.97} \%   &   \bf{66.63} \%   &   \bf{74.26} \%  \\
\bottomrule
\end{tabular}
\caption{Comparing our method with the work of \cite{dong2019multi} (Dong) in reconstruction quality over ten virtual scenes in our dataset. 
}
\label{tab:compare-to-dong-quality}
\end{table}

==> figures/tab_fixed-identities.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cccc}
        \toprule
        \multicolumn{2}{c}{Robot State} & \multirow{2}{*}{T-D(m)} & \multirow{2}{*}{T-C(s)}          \\ \cline{1-2}
        \#\rev{explorer}                & \#\rev{reconstructor}   &                         &        \\ \hline \hline
        1                               & 3                       & 538.74                  & 276.43 \\
        2                               & 2                       & 428.34                  & 406.03 \\
        3                               & 1                       & 317.95                  & 491.93 \\
        \midrule
        \multicolumn{2}{c}{Full}        & \bf{291.45}             & \bf{128.6}                       \\
        \bottomrule
    \end{tabular}
    \caption{Comparing scanning efficiency between our method and fixed-identity situation over 10 virtual scenes. }
    \label{tab:fixed-identities}
\end{table}

==> figures/task-flow-pipeline.tex <==
\begin{figure}[htbp]
\centering

\subfigure[Overview of \textit{task-flow} asynchronous model: 
All robots are processing various tasks. 
Once robot $R_3$ nearly finishes its current task sequence $T_k$, it sends a signal to the control center to generate and assign tasks (TGA). 
The control center will then output the new task sequences and append to each robot's in-progress sequence with the considering of the workload of all robots. 
When robot $R_3$ finishes its current task sequence $T^3_k$, it steps into the identity change state (\textbf{C}) and begins to process new tasks. 
In this way, tasks are being processed by the robots and generated from the control center like a flow. 
]{
\begin{minipage}[t]{0.95\linewidth}
\centering
\includegraphics[width=3.0in]{images/task-flow-pipeline-1.pdf}
%\caption{fig2}
\end{minipage}
}%

\subfigure[This is a close observation of how the robot $R_3$ receives new tasks. 
When task sequence $T_k^3$ is about to be accomplished, the robot signals to the control center. 
The Current accumulated information are gathered and processed to extract two categories of tasks ($\mathcal{T}^E$ and $\mathcal{T}^R$). 
After the analysis of robots' states, the tasks are regrouped into severally sequences and attached to each robot's unfinished tasks. ]{
\begin{minipage}[t]{0.95\linewidth}
\centering
\includegraphics[width=3.0in]{images/task-flow-pipeline-2.pdf}
%\caption{fig2}
\end{minipage}
}%

\centering
\caption{High-level overview of the \textit{task-flow} asynchronous model. And a close observation on the detail of the task-applying process of a single robot. }
\label{fig:task-flow-pipeline}
\end{figure}
